Metric Learning for User-defined Keyword Spotting

The goal of this work is to detect new spoken terms defined by users. While most previous works address Keyword Spotting (KWS) as a closed-set classification problem, this limits their transferability to unseen terms. The ability to define custom keywords has advantages in terms of user experience. In this paper, we propose a metric learning-based training strategy for user-defined keyword spotting. In particular, we make the following contributions: (1) we construct a large-scale keyword dataset with an existing speech corpus and propose a filtering method to remove data that degrade model training; (2) we propose a metric learning-based two-stage training strategy, and demonstrate that the proposed method improves the performance on the user-defined keyword spotting task by enriching their representations; (3) to facilitate the fair comparison in the user-defined KWS field, we propose unified evaluation protocol and metrics. Our proposed system does not require an incremental training on the user-defined keywords, and outperforms previous works by a significant margin on the Google Speech Commands dataset using the proposed as well as the existing metrics.

==> tab/Batch.tex <==
% \begin{table}
%     \centering
%     \begin{tabular}{c|cccc} 
%     \hline
%     \textbf{Batch size} & 32   & 64   & 128  & 256   \\ 
%     \hline
%     \textbf{EER}             & 7.77 & 7.77 & 7.77 & 7.77  \\
%     \hline
%     \end{tabular}
%     \caption{Batch}
% \label{tab:batch}
% \end{table}

\begin{table}
\centering
\begin{tabular}{l|ccccc} 
\hline
B  & EER & Acc & F1-score & FRR@2.5  & FRR@10\\ 
\hline
32      &8.50     &89.28     &0.89          &13.69 &    7.94         \\ 
% \hline
64      &8.96     & 86.81    & 0.87         &  17.31           & 8.08\\ 
% \hline
128     &8.64     & 89.56    &   0.89       &   15.22           &8.11\\
% \hline
256     & 8.39    & 88.56   &   0.88       &     13.61         &7.81\\
\hline
\end{tabular}
\caption{Batch size}
\label{tab:batch}
\end{table}
